Quantum Leak: Timing Side-Channel Attacks on Cloud-Based Quantum Services

Quantum computing offers significant acceleration capabilities over its classical counterpart in various application domains. Consequently, there has been substantial focus on improving quantum computing capabilities. However, to date, the security implications of these quantum computing platforms have been largely overlooked. With the emergence of cloud-based quantum computing services, it is critical to investigate the extension of classical computer security threats to the realm of quantum computing. In this study, we investigated timing-based side-channel vulnerabilities within IBM's cloud-based quantum service. The proposed attack effectively subverts the confidentiality of the executed quantum algorithm, using a more realistic threat model compared to existing approaches. Our experimental results, conducted using IBM's quantum cloud service, demonstrate that with just 10 measurements, it is possible to identify the underlying quantum computer that executed the circuit. Moreover, when evaluated using the popular Grover circuit, we showcase the ability to leak the quantum oracle with a mere 500 measurements. These findings underline the pressing need to address timing-based vulnerabilities in quantum computing platforms and advocate for enhanced security measures to safeguard sensitive quantum algorithms and data.

==> Sections/review.tex <==
\begingroup
%\let\clearpage\relax 
\onecolumn 


\begin{center}
\large {\ul{Reviewer Comments}}

\medskip
\large {\bf Common questions}
\end{center}
%\setstretch{2}

\fontfamily{bch}\selectfont 

\noindent{\bf Q-R1.1: The threat model assumes that the victim's quantum circuit will execute multiple times. Does it mean that the circuit will perform the execution on an input/dataset multiple times, or perform different portions of the computation on a dataset? As the adversary has no control over the victim's dataset, the assumption that he can observe the same computation multiple times seems unrealistic.
}
\noindent{\bf Q-R1.2: Similarly, the paper also mentions that the external attacker can submit a quantum circuit precisely during the overlap of the victim's quantum circuits. How would the attacker know the precise overlap between the victim's circuit, at the beginning of a side-channel attack?
}

\noindent{\bf Q-R2.1: The threat model needs to be revisited. The primary motivation for launching side-channel attacks is to obtain secret information from the computing system, primarily the secret key. Unfortunately, the paper only talks about the identification of underlying circuitry instead of the secret. Why does someone want to protect the circuit? Clearly, the circuit details (a handful of algorithms are currently available in practice, mentioned in Table 1) are known. What information will an adversary gain besides the algorithm you're running on the cloud? Besides, the reviewer thinks the contribution is limited as this is merely an extension of the traditional SCA (using T-test) to quantum circuits. 
}

\noindent{\bf Q-R3.2: To discern the user’s circuit, preliminary data must be collected to establish a baseline for various types of quantum circuits; As per the claims the adversary needs to know preliminary data about each and every circuit variations which might not be feasible considering the large number of quantum circuits and their variations being used.
}

\noindent{\bf Q-R4.3: The timing weaknesses are not that damaging. It doesn't work for the most privacy-sensitive use cases (CA \& QM). In the case of UC and QP, most users wouldn't care if someone knew what well-known quantum algorithms are being run, and the processors are already public information. CO is a somewhat sensitive use case, but the effectiveness of timing attacks is somewhat mixed.
}

\vspace{4pt}
\noindent{\em {\bf A-R1.1,R1.2, R2.1, R3-2, R4.3:} We thank the reviewer for the excellent question.
\vspace{4pt}

\textcolor{black}{In this work, we utilize weaker assumptions compared to the prior work, thus, making it more realistic, and reducing the capabilities of the attacker.} Specifically, unlike \cite{ccspscaquantum}, we do not assume the attacker has physical access to power measurement~\cite{ccspscaquantum, quantumcloudsca}. Our assumptions of the attacker's available resources are listed as follows:
\begin{itemize}
%\itemsep0em
\item \textcolor{black}{The victim's circuit with the same operations is executed multiple times, similar to~\cite{ccspscaquantum,quantumcloudsca}.}
\item The attack can measure timing for each execution of a circuit~\cite{ccspscaquantum}. Note this is a more realistic assumption than in~\cite{ccspscaquantum} where the adversary can have physical access to measure power.
\item The attacker circuit can be executed during two executions of the two victim circuit execuitons~\cite{quantumcloudsca}.
\item \textcolor{black}{The attacker does not require power, or energy properties for each execution of a circuit, nor access to the qubit drive equipment, where the attacker can collect power and energy traces from the arbitrary waveform generator or the mixer, as was assumed in~\cite{ccspscaquantum}.} 
\item We assume that consecutive executions do not affect the overall time consumption of the quantum circuits, even though the system might take longer to cool down.
\item The randomness of the compilation strategy should be eliminated, meaning that with each compilation of the quantum circuit, the qubit mapping and routing path remain fixed, which is a hidden assumption in~\cite{ccspscaquantum}.
\item The timing SCA encompasses the entire pulse wave preparation stage, comprising digital processing, analog processing, and quantum processing stages, as depicted in Figure~\ref{fig:quantumarch} as the quantum processing unit. The omission of classical processing is due to the relatively shorter time consumption in each computation cycle compared with the other portions of the computation.
\end{itemize}

Note that in cases where multiple victim circuit executions occur between two attacker circuit executions, the attacker can estimate the equal time consumption for each victim execution by comparing it with the average time consumption for the victim's circuit. For example, if the average time consumption for the measured victim's circuit is 3 seconds and the time difference between two quantum circuit measurements from the attacker is 9.1 seconds, the attacker can infer that there were approximately three executions of the victim's circuit between the two measurements of the attacker circuits. This is addressed in Section~\ref{sec:Methodology}
of the paper.

}

\medskip
\noindent{\bf Q-R1.4: There are a few typos/grammatical errors in the manuscript. For example, (i) Hadardmard instead of Hadamard, (ii) Reconstruction from Power Traces (caps not required for the first letter).
}

\noindent{\bf Q-R2.2: The paper requires comprehensive proofreading. In one instance, the authors assert that there is limited research on security for quantum circuits, while in another section, they indicate that considerable effort has been dedicated to this area.
}

\vspace{4pt}
\noindent{\em {\bf A-R1.4, 2.2:} We have proofread the paper and fixed the typos and grammatical errors to improve the readability of the paper.

}

\medskip

\begin{center}
\large {\bf Reviewer 1}
\end{center}

\noindent{\bf Q-R1.1: The threat model assumes that the victim's quantum circuit will execute multiple times. Does it mean that the circuit will perform the execution on an input/dataset multiple times, or perform different portions of the computation on a dataset? As the adversary has no control over the victim's dataset, the assumption that he can observe the same computation multiple times seems unrealistic. Similarly, the paper also mentions that the external attacker can submit a quantum circuit precisely during the overlap of the victim's quantum circuits. How would the attacker know the precise overlap between the victim's circuit, at the beginning of a side-channel attack?
}

\vspace{4pt}
\noindent{\em {\bf A-R1.1:} We thank the reviewer for the excellent question.
\vspace{4pt}

\textcolor{black}{In this work, we utilize weaker assumptions compared to the prior work, thus, making it more realistic, and reducing the capabilities of the attacker.} Specifically, unlike \cite{ccspscaquantum}, we do not assume the attacker has physical access to power measurement~\cite{ccspscaquantum, quantumcloudsca}. Our assumptions of the attacker's available resources are listed as follows:
\begin{itemize}
%\itemsep0em
\item \textcolor{black}{The victim's circuit with the same operations is executed multiple times, similar to~\cite{ccspscaquantum,quantumcloudsca}.}
\item The attack can measure timing for each execution of a circuit~\cite{ccspscaquantum}. Note this is a more realistic assumption than in~\cite{ccspscaquantum} where the adversary can have physical access to measure power.
\item The attacker circuit can be executed during two executions of the two victim circuit execuitons~\cite{quantumcloudsca}.
\item \textcolor{black}{The attacker does not require power, or energy properties for each execution of a circuit, nor access to the qubit drive equipment, where the attacker can collect power and energy traces from the arbitrary waveform generator or the mixer, as was assumed in~\cite{ccspscaquantum}.} 
\item We assume that consecutive executions do not affect the overall time consumption of the quantum circuits, even though the system might take longer to cool down.
\item The randomness of the compilation strategy should be eliminated, meaning that with each compilation of the quantum circuit, the qubit mapping and routing path remain fixed, which is a hidden assumption in~\cite{ccspscaquantum}.
\item The timing SCA encompasses the entire pulse wave preparation stage, comprising digital processing, analog processing, and quantum processing stages, as depicted in Figure~\ref{fig:quantumarch} as the quantum processing unit. The omission of classical processing is due to the relatively shorter time consumption in each computation cycle compared with the other portions of the computation.
\end{itemize}

Note that in cases where multiple victim circuit executions occur between two attacker circuit executions, the attacker can estimate the equal time consumption for each victim execution by comparing it with the average time consumption for the victim's circuit. For example, if the average time consumption for the measured victim's circuit is 3 seconds and the time difference between two quantum circuit measurements from the attacker is 9.1 seconds, the attacker can infer that there were approximately three executions of the victim's circuit between the two measurements of the attacker circuits. This is addressed in Section~\ref{sec:Methodology}
of the paper.



}


\medskip
\noindent{\bf Q-R1.3: The paper talks about potential defense mechanisms. Wouldn't a simple randomization of the victim's quantum circuit execution order during runtime thwart/complicate the proposed attack?
}

\vspace{4pt}
\noindent{\em {\bf A-R1.3:} 
While we acknowledge that randomizing the execution order of the victim's quantum circuit during runtime has the potential to thwart the proposed attack, we assert the importance of persuading the community about the feasibility of such an attack in obtaining private information when these protective measures are not implemented within the cloud service. This is addressed in Section~\ref{sec:Methodology} of the paper.

}
\medskip
\noindent{\bf Q-R1.4: There are a few typos/grammatical errors in the manuscript. For example, (i) Hadardmard instead of Hadamard, (ii) Reconstruction from Power Traces (caps not required for the first letter).
}

\vspace{4pt}
\noindent{\em {\bf A-R1.4:} We have proofread the paper and fixed the typos and grammatical errors to improve the readability of the paper.

}
\medskip
\begin{center}
\large {\bf Reviewer 2}
\end{center}

\noindent{\bf Q-R2.1: The threat model needs to be revisited. The primary motivation for launching side-channel attacks is to obtain secret information from the computing system, primarily the secret key. Unfortunately, the paper only talks about the identification of underlying circuitry instead of the secret. Why does someone want to protect the circuit? Clearly, the circuit details (a handful of algorithms are currently available in practice, mentioned in Table 1) are known. What information will an adversary gain besides the algorithm you're running on the cloud? Besides, the reviewer thinks the contribution is limited as this is merely an extension of the traditional SCA (using T-test) to quantum circuits. 
}

\vspace{4pt}
\noindent{\em {\bf A-R2.1:} We thank the reviewer for the excellent question.
\vspace{4pt}

\textcolor{black}{In this work, we utilize weaker assumptions compared to the prior work, thus, making it more realistic, and reducing the capabilities of the attacker.} Specifically, unlike \cite{ccspscaquantum}, we do not assume the attacker has physical access to power measurement~\cite{ccspscaquantum, quantumcloudsca}. Our assumptions of the attacker's available resources are listed as follows:
\begin{itemize}
%\itemsep0em
\item \textcolor{black}{The victim's circuit with the same operations is executed multiple times, similar to~\cite{ccspscaquantum,quantumcloudsca}.}
\item The attack can measure timing for each execution of a circuit~\cite{ccspscaquantum}. Note this is a more realistic assumption than in~\cite{ccspscaquantum} where the adversary can have physical access to measure power.
\item The attacker circuit can be executed during two executions of the two victim circuit execuitons~\cite{quantumcloudsca}.
\item \textcolor{black}{The attacker does not require power, or energy properties for each execution of a circuit, nor access to the qubit drive equipment, where the attacker can collect power and energy traces from the arbitrary waveform generator or the mixer, as was assumed in~\cite{ccspscaquantum}.} 
\item We assume that consecutive executions do not affect the overall time consumption of the quantum circuits, even though the system might take longer to cool down.
\item The randomness of the compilation strategy should be eliminated, meaning that with each compilation of the quantum circuit, the qubit mapping and routing path remain fixed, which is a hidden assumption in~\cite{ccspscaquantum}.
\item The timing SCA encompasses the entire pulse wave preparation stage, comprising digital processing, analog processing, and quantum processing stages, as depicted in Figure~\ref{fig:quantumarch} as the quantum processing unit. The omission of classical processing is due to the relatively shorter time consumption in each computation cycle compared with the other portions of the computation.
\end{itemize}

Note that in cases where multiple victim circuit executions occur between two attacker circuit executions, the attacker can estimate the equal time consumption for each victim execution by comparing it with the average time consumption for the victim's circuit. For example, if the average time consumption for the measured victim's circuit is 3 seconds and the time difference between two quantum circuit measurements from the attacker is 9.1 seconds, the attacker can infer that there were approximately three executions of the victim's circuit between the two measurements of the attacker circuits.
This is addressed in Section~\ref{sec:Methodology} of the paper.



}
\medskip
\noindent{\bf Q-R2.2: The paper requires comprehensive proofreading. In one instance, the authors assert that there is limited research on security for quantum circuits, while in another section, they indicate that considerable effort has been dedicated to this area.
}

\vspace{4pt}
\noindent{\em {\bf A-R2.2:} We have proofread the paper and fixed the typos and grammatical errors to improve the readability of the paper.

}
\medskip
\noindent{\bf Q-R2.3: The paper's structure requires significant refinement. The first four pages are dedicated to the introduction and background, leaving only one page for the proposed methodology (section IV), which, in my opinion, is insufficient.
}

\noindent{\em {\bf A-R2.3:} We introduce more details with the threat model with detailed assumptions in Section~\ref{sec:Methodology}. 

}
\medskip
\begin{center}
\large {\bf Reviewer 3}
\end{center}

\noindent{\bf Q-R3.1: The adversary calculates the execution time of the victim circuit by determining the time interval between the start time of the second job and the end time of the first job. It is assumed that this calculated time closely approximates the actual execution time of the victim circuit. However, this assumption might not hold true. 
This is addressed in Section~\ref{sec:Methodology} of the paper.

}

\vspace{4pt}
\noindent{\em {\bf A-R3.1:} We thank the reviewer for the excellent question.
\vspace{4pt}


We believe that the major difference in the time consumption is during the quantum processor phase. The other classical elements have minor differences that can be considered as constant time consumption, which are minimal compared with the quantum circuit execution. 
Neglecting the interval between the executions of two quantum circuits allows us to create a timing trace for different executions without considering the time elapsed between them. In cases where the time consumption varies between two executions but remains consistent within each run, recovering the initial timing data becomes seamless. This is accomplished by subtracting the total time consumption during two consecutive executions.

}
\medskip
\noindent{\bf Q-R3.2: To discern the user’s circuit, preliminary data must be collected to establish a baseline for various types of quantum circuits; As per the claims the adversary needs to know preliminary data about each and every circuit variation which might not be feasible considering the large number of quantum circuits and their variations being used.
}

\vspace{4pt}
\noindent{\em {\bf A-R3.2:} \textcolor{black}{In this work, we utilize weaker assumptions compared to the prior work, thus, making it more realistic, and reducing the capabilities of the attacker.} Specifically, unlike \cite{ccspscaquantum}, we do not assume the attacker has physical access to power measurement~\cite{ccspscaquantum, quantumcloudsca}. Our assumptions of the attacker's available resources are listed as follows:
\begin{itemize}
%\itemsep0em
\item \textcolor{black}{The victim's circuit with the same operations is executed multiple times, similar to~\cite{ccspscaquantum,quantumcloudsca}.}
\item The attack can measure timing for each execution of a circuit~\cite{ccspscaquantum}. Note this is a more realistic assumption than in~\cite{ccspscaquantum} where the adversary can have physical access to measure power.
\item The attacker circuit can be executed during two executions of the two victim circuit execuitons~\cite{quantumcloudsca}.
\item \textcolor{black}{The attacker does not require power, or energy properties for each execution of a circuit, nor access to the qubit drive equipment, where the attacker can collect power and energy traces from the arbitrary waveform generator or the mixer, as was assumed in~\cite{ccspscaquantum}.} 
\item We assume that consecutive executions do not affect the overall time consumption of the quantum circuits, even though the system might take longer to cool down.
\item The randomness of the compilation strategy should be eliminated, meaning that with each compilation of the quantum circuit, the qubit mapping and routing path remain fixed, which is a hidden assumption in~\cite{ccspscaquantum}.
\item The timing SCA encompasses the entire pulse wave preparation stage, comprising digital processing, analog processing, and quantum processing stages, as depicted in Figure~\ref{fig:quantumarch} as the quantum processing unit. The omission of classical processing is due to the relatively shorter time consumption in each computation cycle compared with the other portions of the computation.
\end{itemize}

Note that in cases where multiple victim circuit executions occur between two attacker circuit executions, the attacker can estimate the equal time consumption for each victim execution by comparing it with the average time consumption for the victim's circuit. For example, if the average time consumption for the measured victim's circuit is 3 seconds and the time difference between two quantum circuit measurements from the attacker is 9.1 seconds, the attacker can infer that there were approximately three executions of the victim's circuit between the two measurements of the attacker circuits. This is addressed in Section~\ref{sec:Methodology} of the paper.




}
\medskip
\begin{center}
\large {\bf Reviewer 4}
\end{center}

\noindent{\bf Q-R4.1: The paper requires strict, almost non-realistic assumptions in a deployed cloud-based quantum system, such as being able to isolate the quantum processor timing from the classical and digital timers.
}

\vspace{4pt}
\noindent{\em {\bf A-R4.1:} We thank the reviewer for the excellent question.
\vspace{4pt}
We believe that the major difference in the time consumption is during the quantum processor phase. The other classical elements have minor differences that can be considered as constant time consumption, which are minimal compared with the quantum circuit execution. 
Neglecting the interval between the executions of two quantum circuits allows us to create a timing trace for different executions without considering the time elapsed between them. In cases where the time consumption varies between two executions but remains consistent within each run, recovering the initial timing data becomes seamless. This is accomplished by subtracting the total time consumption during two consecutive executions. This is addressed in Section~\ref{sec:Methodology} of the paper.



}
\medskip
\noindent{\bf Q-R4.2: The applicability of the attacks is speculative since there aren't practical quantum computers yet available.
}



\vspace{4pt}
\noindent{\em {\bf A-R4.1:} Indeed, the applicability of attacks is speculative AND this is why we need to explore it now, as we are developing these systems instead of treating it as an afterthought. The whole emerging field of quantum computer security with recent papers at top venues like CCS~\cite{ccspscaquantum}, S\&P, and HOST~\cite{deshpande2022towards} is exploring such speculative attacks.
This is addressed in Section~\ref{sec:related} of the paper.

}

\medskip
\noindent{\bf Q-R4.3: The timing weaknesses are not that damaging. It doesn't work for the most privacy-sensitive use cases (CA \& QM). In the case of UC and QP, most users wouldn't care if someone knew what well-known quantum algorithms are being run, and the processors are already public information. CO is a somewhat sensitive use case, but the effectiveness of timing attacks is somewhat mixed.
}

\vspace{4pt}
\noindent{\em {\bf A-R1.1:} \textcolor{black}{In this work, we utilize weaker assumptions compared to the prior work, thus, making it more realistic, and reducing the capabilities of the attacker.} Specifically, unlike \cite{ccspscaquantum}, we do not assume the attacker has physical access to power measurement~\cite{ccspscaquantum, quantumcloudsca}. Our assumptions of the attacker's available resources are listed as follows:
\begin{itemize}
%\itemsep0em
\item \textcolor{black}{The victim's circuit with the same operations is executed multiple times, similar to~\cite{ccspscaquantum,quantumcloudsca}.}
\item The attack can measure timing for each execution of a circuit~\cite{ccspscaquantum}. Note this is a more realistic assumption than in~\cite{ccspscaquantum} where the adversary can have physical access to measure power.
\item The attacker circuit can be executed during two executions of the two victim circuit execuitons~\cite{quantumcloudsca}.
\item \textcolor{black}{The attacker does not require power, or energy properties for each execution of a circuit, nor access to the qubit drive equipment, where the attacker can collect power and energy traces from the arbitrary waveform generator or the mixer, as was assumed in~\cite{ccspscaquantum}.} 
\item We assume that consecutive executions do not affect the overall time consumption of the quantum circuits, even though the system might take longer to cool down.
\item The randomness of the compilation strategy should be eliminated, meaning that with each compilation of the quantum circuit, the qubit mapping and routing path remain fixed, which is a hidden assumption in~\cite{ccspscaquantum}.
\item The timing SCA encompasses the entire pulse wave preparation stage, comprising digital processing, analog processing, and quantum processing stages, as depicted in Figure~\ref{fig:quantumarch} as the quantum processing unit. The omission of classical processing is due to the relatively shorter time consumption in each computation cycle compared with the other portions of the computation.
\end{itemize}

Note that in cases where multiple victim circuit executions occur between two attacker circuit executions, the attacker can estimate the equal time consumption for each victim execution by comparing it with the average time consumption for the victim's circuit. For example, if the average time consumption for the measured victim's circuit is 3 seconds and the time difference between two quantum circuit measurements from the attacker is 9.1 seconds, the attacker can infer that there were approximately three executions of the victim's circuit between the two measurements of the attacker circuits. This is addressed in Section~\ref{sec:Methodology} of the paper.



}
